The quantization of a toric manifold is given by the integer lattice points in the moment polytope

We describe a very nice argument, which we learned from Sue Tolman, that the dimension of the quantization space of a toric manifold, using a Kaehler polarization, is given by the number of integer lattice points in the moment polytope.

==> head.tex <==
%% This is yet a third version of the ``head'' file,
%% intended to be a general-purpose file.
%% This should now be the standard "head" reference file, superseding
%% the one in the thesis/ directory.
%% However, it is not entirely clear what should be in here or not.
%% Perhaps each document should have its own file?
%% Perhaps each document should have all its commands in the preamble?
%%
%% I think we should have one place (here) where ALL commands are listed;
%% we can create special sections for specific files if that seems like
%% a good idea.
%% So that's the plan.

% Last updated 18 July 2007

%Sets
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\cp}{\mathbb{C}P^1}	 
\newcommand{\st}{\mid}  % "such that" in set-builder notation--can be chg'd
%Vectors
\newcommand{\ii}{\mathbf{i}}
\newcommand{\jj}{\mathbf{j}}
\newcommand{\kk}{\mathbf{k}}
\newcommand{\rr}{\mathbf{r}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\ww}{\mathbf{w}}
\newcommand{\uu}{\mathbf{u}}
\newcommand{\ee}{\mathbf{e}}
\newcommand{\xx}{\mathbf{x}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}

%Operators & Operations
\newcommand{\del}{\partial}
\newcommand{\dbar}{\bar{\partial}}
\newcommand{\restr}[1]{\bigr\rvert_{#1}}
\newcommand{\cross}{\times}
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\ip}[2]{\langle#1,#2\rangle}	% inner product--may be changed
\newcommand{\tensor}{\otimes}

%Calculus
\newcommand{\dd}[2]{\frac{\del #1}{\del #2}}   %general partial derivative
\newcommand{\dydx}{\frac{dy}{dx}} %total derivative
\newcommand{\grad}{\boldsymbol{\nabla}}
\newcommand{\jactwo}[4]{\frac{\del(#1,#2)}{\del(#3,#4)}}  %Jacobians
\newcommand{\jacthree}[6]{\frac{\del(#1,#2,#3)}{\del(#4,#5,#6)}}
\newcommand{\hess}{\mathcal{H}}  %Hessian

%Exposition
\newcommand{\note}[1]{\emph{Note: #1}}
\newcommand{\andso}{\quad\rightsquigarrow\quad}
\newcommand{\define}[1]{\textsl{#1}}
\newcommand{\dadum}[1]{\vspace{1ex} \noindent \textbf{#1}} % emphasis
\newcommand{\gap}{\vspace{2ex}}

%Miscellaneous math
\newcommand{\Lie}[1]{\mathfrak{#1}}	%% Lie algebra
\newcommand{\into}{\hookrightarrow}
\newcommand{\pb}{^*\!}  % "pullback"
\newcommand{\inv}{^{-1}} % "inverse"
\newcommand{\actson}{\circlearrowleft} % group acting on...

% Somewhat more obscure; not sure if necessary
\newcommand{\ddx}[2]{\frac{\del #2}{\del x_{#1}}}    %ddx with subscripts
\newcommand{\ddy}[2]{\frac{\del #2}{\del y_{#1}}}    %ddy with subscripts

% Lazy typing
\newcommand{\nbhd}{neighbourhood}
\newcommand{\w}{\omega}	  %lazy man's symplectic form

%Other
\newcommand{\disp}{\displaystyle}  %used for in-line presentations of integrals

%Theorems--uncomment as necessary
\theoremstyle{definition}
\newtheorem{thm}{Theorem}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{claim}[thm]{Claim}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{defnn}[thm]{Definition}
\newtheorem*{defn}{Definition}
\newtheorem*{notn}{Notation}	
\newtheorem*{rmk}{Remark}
\newtheorem*{mprop}{Major Proposition}
\newtheorem*{thmm}{Main Theorem}
\newtheorem*{thmn}{Theorem}
\newtheorem*{lemn}{Lemma}
\newtheorem*{claimn}{Claim}
\newtheorem{fact}{Fact}
\theoremstyle{remark}
\newtheorem*{eg}{Example}
\newtheorem{ex}{Exercise}

%Formatting for epigraphs (from thesis) --- arguments are {text}{author},
% with {text} formatted using verse formatting, ie \\ for line break
\newcommand{\epigraph}[2]{\begin{verse}\small{\it #1}\\ 
\hspace{5em} --- #2 \end{verse}}



%\renewcommand{\thefootnote}{\ensuremath{\fnsymbol{footnote}}}

%Puts the date at the top of each page
\pagestyle{myheadings}
\markright{\scriptsize \today}




